Moduli spaces of stable pairs and non-abelian zeta functions of curves via wall-crossing

In this paper we study and relate the non-abelian zeta functions introduced by Weng and invariants of the moduli spaces of arbitrary rank stable pairs over curves. We prove a wall-crossing formula for the latter invariants and obtain an explicit formula for these invariants in terms of the motive of a curve. Previously, formulas for these invariants were known only for rank 2 due to Thaddeus and for rank 3 due to Mu\~noz. Using these results we obtain an explicit formula for the non-abelian zeta functions, we check the uniformity conjecture by Weng for the ranks 2 and 3, and we prove the counting miracle conjecture.

==> commands.tex <==
\RequirePackage{amsmath,amssymb,xspace}


\theoremstyle{plain}
\newtheorem{nthr}{Theorem}[section]
\newtheorem{theorem}		[nthr]{Theorem}
\newtheorem{proposition}[nthr]{Proposition}
\newtheorem{lemma}		[nthr]{Lemma}
\newtheorem{corollary}	[nthr]{Corollary}
\newtheorem{claim}		[nthr]{Claim}
\newtheorem{conjecture} [nthr]{Conjecture}
\newtheorem{remark}		[nthr]{Remark}
\theoremstyle{definition}
\newtheorem{definition} [nthr]{Definition}
\newtheorem{example}		[nthr]{Example}

\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\oper#1#2{\dmat#1{\operatorname{#2}}}

\dmat\bk{\Bbbk}
\dmat\bA{\mathbb{A}}
\dmat\bC{\mathbb{C}}
\dmat\bF{\mathbb{F}}
\dmat\bG{\mathbb{G}}
\dmat\bH{\mathbb{H}}
\dmat\bL{\mathbb{L}}
\dmat\bN{\mathbb{N}}
\dmat\bQ{\mathbb{Q}}
\dmat\bP{\mathbb{P}}
\dmat\bR{\mathbb{R}}
\dmat\bT{\mathbb{T}}
\dmat\bZ{\mathbb{Z}}
\dmat\cA{\mathcal{A}}
\dmat\cC{\mathcal{C}}
\dmat\cF{\mathcal{F}}
\dmat\cG{\mathcal{G}}
\dmat\cM{\mathcal{M}}
\dmat\cO{\mathcal{O}}
\dmat\cP{\mathcal{P}}
\dmat\cS{\mathcal{S}}
\dmat\cT{\mathcal{T}}
\dmat\cU{\mathcal{U}}
\dmat\cV{\mathcal{V}}
\dmat\cZ{\mathcal{Z}}
\dmat\bfM{\mathbf{M}}

\dmat\al\alpha
\dmat\be\beta
\dmat\ga\gamma
\dmat\de\delta
\dmat\eps{\varepsilon}
\dmat\hi\chi
\dmat\vi\varphi
\dmat\te\theta
\dmat\ka\kappa
\dmat\si\sigma
\dmat\Ga\Gamma
\dmat\Om\Omega
\dmat\ta{\tau}
\dmat\om{\omega}
\dmat\la{\lambda}

\def\ang#1{\mat{\left\langle #1\right\rangle}}
\def\angs#1#2{\mat{\left\langle #1 \mid #2\right\rangle}}
\def\set#1{\mat{\{#1\}}}
\def\sets#1#2{\mat{\{#1\mid#2\}}}
\def\case#1{\begin{cases}#1\end{cases}}
\def\rbr#1{\left(#1\right)}
\def\sbr#1{\left[#1\right]}
\def\sb{\subset}
\def\ms{\backslash}
\def\ts{\otimes}
\dmat\oh{\frac12}
\dmat\Gm{{\bG_{\mathrm m}}}
\def\what#1{\mat{\widehat{#1}}}

\def\inv{^{-1}}
\def\vir{{\mathrm{vir}}}
\def\n#1{\mat{\lvert#1\rvert}}
\def\nn#1{\mat{\lVert#1\rVert}}
\def\ie{i.e.\ }
\def\mto{\mapsto}
\def\lb#1{\mat{\underline{#1}}} %lower bar
\def\ub#1{\mat{\overline{#1}}}  %upper bar
\def\udim{\lb\dim}
\def\bop{\bigoplus}
\def\pser#1{[\![#1]\!]} %formal power series [[#1]]
\def\lser#1{\mbox{(\!(}#1\mbox{)\!)}} %formal Laurent series ((#1))
\def\xx{\times}
\def\iso{\simeq}
\def\over#1#2{\mat{\substack{#1\\#2}}} % #2 over #1
\dmat\es{\varnothing}
\def\arr^#1{\xrightarrow{#1}}
\def\ind{\mathrm{ind}}
\def\df{^\mathrm{def}}
\dmat\iff\Leftrightarrow
\def\st{\mathrm{st}}
\def\lqq{\lq\lq}
\def\rqq{\rq\rq\xspace}


\oper\Var{Var}
\oper\Hom{Hom}
\oper\Ext{Ext}
\oper\GL{GL}
\oper\supp{supp}
\oper\End{End}
\oper\Iso{Iso}
\oper\ch{ch}
\oper\cl{cl}
\oper\Aut{Aut}
\oper\Coh{Coh}
\oper\rk{rk}
\oper\coker{coker}
\oper\Hilb{Hilb}
\oper\im{im}
\oper\Exp{Exp}
\oper\Jac{Jac}
\oper\Bun{Bun}
\oper\Pow{Pow}
\oper\SL{SL}
\oper\Log{Log}

\newif\ifrem\remtrue
\def\rem#1{\ifrem\marginpar{\raggedright\footnotesize #1}\fi}
\def\eq#1{\begin{equation}#1\end{equation}}
\def\eql#1#2{\begin{equation}#1\label{#2}\end{equation}}
\def\one{\mathbf 1}
\def\sst{\mathrm{sst}}
\def\coeff{\operatorname{\mathsf{coeff}}}
\def\sb{\subset}
\def\flr#1{\left\lfloor#1\right\rfloor}
\def\ceil#1{\left\lceil#1\right\rceil}

